A Lightweight and Accurate Spatial-Temporal Transformer for Traffic Forecasting

We study the forecasting problem for traffic with dynamic, possibly periodical, and joint spatial-temporal dependency between regions. Given the aggregated inflow and outflow traffic of regions in a city from time slots 0 to t-1, we predict the traffic at time t at any region. Prior arts in the area often consider the spatial and temporal dependencies in a decoupled manner or are rather computationally intensive in training with a large number of hyper-parameters to tune. We propose ST-TIS, a novel, lightweight, and accurate Spatial-Temporal Transformer with information fusion and region sampling for traffic forecasting. ST-TIS extends the canonical Transformer with information fusion and region sampling. The information fusion module captures the complex spatial-temporal dependency between regions. The region sampling module is to improve the efficiency and prediction accuracy, cutting the computation complexity for dependency learning from $O(n^2)$ to $O(n\sqrt{n})$, where n is the number of regions. With far fewer parameters than state-of-the-art models, the offline training of our model is significantly faster in terms of tuning and computation (with a reduction of up to $90\%$ on training time and network parameters). Notwithstanding such training efficiency, extensive experiments show that ST-TIS is substantially more accurate in online prediction than state-of-the-art approaches (with an average improvement of up to $9.5\%$ on RMSE, and $12.4\%$ on MAPE).

==> 6_case_study.tex <==
\section{Case studies}
\label{sec:case_study}

In this section, we present some case studies to demonstrate that \modelname{} is interpretable and effective for capturing the region correlations, temporal dependencies, and irregularity effect. We study the region correlations in Section~\ref{sec: region correlation study}, and the temporal dependencies and irregularity effect in Section~\ref{sec:temporal dependency and anomily effect}. 


             
%It is intuitively that the volume of transition between two regions reflects their correlation. Transition data have been widely used to predict the traffic demand for ride-hailing service. 
%However, it is not always available for some scenarios. For example, the inflow and outflow data of a intersection can be collected by deploying sensors on the roads, but transition data between intersection is difficult to collected. 

\subsection{Region correlation study}
\label{sec: region correlation study}




Recall that the correlation between regions is represented as the attention score in the region attention model. We discuss the following questions by visualizing the attention scores between regions:
\begin{itemize}
    \item Is the correlation between two regions inversely proportionate to their distance as assumed in many prior works?
    \item Without using transition data, can \FRAMEWORK{} capture the dependency regarding transition between regions?
\end{itemize}



%Intuitively, the spatial correlation between two regions should be highly correlated with their transition data. Thus, we use heatmaps to visualize and compare the spatial correlation and the transition data. Furthermore, we use the Student T-test and Pearson correlation to evaluate the correlation between the learned spatial correlation and the transition data.

The taxi dataset is used for the following discussion. Following the experimental setting, the whole city is partitioned into $10 \times 20$ regions, where $(a,b)$ denotes the region at the $a$-th row and $b$-th column. Given a region $\hat{r}$ and a time slot $t$, we use the score $\alpha_m(\hat{r},r_i,t)$~(Equation $5$) to represent the influence from $r_i$ to $\hat{r}$~(i.e., in-influence), and $\alpha_m(r_i,\hat{r},t)$ to represent the influence from $\hat{r}$ to $r_i$~(i.e., out-influence). We select the region at $(4,6)$ as $\hat{r}$, and visualize the out-influence and in-influence at the time slot 20:00 - 20:30 at one day in Figures \ref{fig:out_influence} and \ref{fig:in_influence}.  Meanwhile, we visualize the transition from $\hat{r}$ to other regions~(i.e., out-transition) in Figure \ref{fig:out_transition} and the transition from other regions to $\hat{r}$~(i.e., in-transition) at the same time slot in Figure \ref{fig:in_transition}. In the figures, dark colors indicate a large influence. Note that the bike dataset has similar results, but we do not present the results here because of the page limitation.

\begin{figure}
    \noindent\makebox[\linewidth][c]{
        \subfigure[\small Out-influence.]{
            \label{fig:out_influence}
            \includegraphics[width=0.24\textwidth]{./figure/outflow_attention_t_8_l_4_6.png}
        }
        %\vspace{.6in}
        \subfigure[\small Out-transition.]{
            \label{fig:out_transition}
            \includegraphics[width=0.24\textwidth]{./figure/outflow_volume_t_8_l_4_6.png}
        }
    }
    \caption{Comparison of out-influence and out-transition.}
    \label{fig:comparision_of_out}
    \end{figure}


\begin{figure}
    \noindent\makebox[\linewidth][c]{
        \subfigure[\small In-influence.]{
            \label{fig:in_influence}
            \includegraphics[width=0.24\textwidth]{./figure/inflow_attention_t_8_l_4_6.png}
        }
        %\vspace{.6in}
        \subfigure[\small In-transition.]{
            \label{fig:in_transition}
            \includegraphics[width=0.24\textwidth]{./figure/inflow_volume_t_8_l_4_6.png}
        }
    }
    \caption{Comparison of in-influence and in-transition.}
    \label{fig:comparison_of_in}
    \end{figure}



    
    \begin{table}
        \centering
        \caption{Correlation evaluation.}
        
        \begin{tabular}{cccll}
        
        \cline{1-3}
        \multicolumn{1}{|l|}{}                                  & \multicolumn{1}{c|}{P-value} & \multicolumn{1}{c|}{$\rho$} &  &  \\ \cline{1-3}
        \multicolumn{1}{|c|}{In-influence vs. In-transition}   & \multicolumn{1}{c|}{0.0059}        & \multicolumn{1}{c|}{0.8862}            &  &  \\ \cline{1-3}
        \multicolumn{1}{|c|}{Out-influence vs. Out-transition} & \multicolumn{1}{c|}{0.0241}        & \multicolumn{1}{c|}{0.9059
        }            &  &  \\ \cline{1-3}
                                                                &                              &                                  &  & 
        \end{tabular}
        \label{table:correlation}
        \end{table}
        
 

As shown in Figure \ref{fig:out_influence}, close regions do not guarantee higher correlation than distant regions. For example, the region $(4,5)$ is closer to the target region $(4,6)$ than the regions $(2,5)$ and $(2,6)$, but the color of $(2,5)$ and $(2,6)$ is darker than $(4,5)$, indicating that $(2,5)$ and $(2,6)$ have higher correlations with $(4,6)$ than $(4,5)$. Similar results can be found in Figure \ref{fig:in_influence}. The results demonstrate that the correlation between two regions does not have to be inversely proportionate to their distance as assumed in many prior works, and it is crucial to learn the correlation using data-driven approach as we do in this work. 


Furthermore, as shown in Figure \ref{fig:comparision_of_out}, the heatmap of the out-influence is similar to that of the out-transition. In Figure \ref{fig:out_transition}, the region at $(5,8)$ has a significant influence on $\hat{r}$, which can also be found in Figure \ref{fig:out_influence}. Even small influences from a distant region can be captured in Figure \ref{fig:out_influence}, such as the regions at $(0,0)$ and $(1,0)$.  The heatmap of in-influence and in-transition in Figure \ref{fig:comparison_of_in} also leads to similar findings. The visualization results show that our model is interpretable and effective for learning correlations between regions. 

%Furthermore, we use the Student T-test and Pearson correlation to evaluate the correlation between the learned influence and transition. 
Moreover, we then use the Student T-test and Pearson correlation to evaluate the correlation between the attention scores and the transition data. The evaluation results of the P-value and the Pearson correlation coefficients $\rho$ are presented in Table \ref{table:correlation}. Since the P-value is small~($< 0.01$) and $\rho$ is close to $1$, the learned influence is highly correlated with the transition data, which demonstrates the effectiveness of our proposed model to capture the influence between regions. Even without transition data, \FRAMEWORK{} can still learn the correlation between regions regarding their underlying transition.


\subsection{Temporal dependency and irregularity effect study}
\label{sec:temporal dependency and anomily effect}


Recall that we use a temporal attention module to learn the dependency between the predicted time slot and any historical time slot. We visualize the temporal dependency~(i.e., attention scores in TAM) by heatmaps to study the following questions:
\begin{itemize}
    \item Does the temporal dependency vary for different regions even at the same slot?
    \item Does the temporal dependency vary for the same region at different times-of-day or on different days?
    \item Can the temporal attention module capture the irregularity effect?
\end{itemize} 

%\begin{figure}%[!t]
%    \centering
%    \includegraphics[width=0.65\linewidth]{./figure/temporal_dependency_different_region.png}
%    \caption{Temporal dependency of different regions at a time slot.}
%    \label{fig:different_region}
%  \end{figure}

We first present the temporal dependency of ten regions~(regions $(2,\ell)$ where $\ell = 10,11,\cdots 19$) at the same time slot~(20:00 - 20:30) in Figure \ref{fig:different_region}. The x-axis is the $16$ historical time slots, in which $0 \sim 5$ is the past $6$ time slots for short-term dependency, $6 \sim 11$ is the same time slot in the recent past $6$ days, and $12 \sim 15$ is the same time slot on the same day-of-week for the past $4$ weeks. The y-axis is ten regions. A cell $(x_i, y_i)$ denotes the dependency of region $y_i$ on the time slot $x_i$. A dark color represents prominent dependency. From Figure \ref{fig:different_region}, we find that the temporal dependency varies for different regions even at the same slot. It is because distinct regions may have distinct traffic patterns and hence have different dependencies on the historical time slots. The results indicate that \FRAMEWORK{} can capture the dynamic temporal dependencies for different regions. 


%\begin{figure}%[!t]
%    \centering
%    \includegraphics[width=0.65\linewidth]{./figure/temporal_dependency_different_day.png}
%    \caption{Temporal dependency of a region at different days.}
%    \label{fig:different day}
%  \end{figure}


  \begin{figure}
    \noindent\makebox[\linewidth][c]{
        \subfigure[Different regions at a time slot.]{
            \label{fig:different_region}
            \includegraphics[width=0.25\textwidth]{./figure/temporal_dependency_different_region.png}
        }
        \vspace{.6in}
        \subfigure[A region on different days.]{
            \label{fig:different day}
            \includegraphics[width=0.25\textwidth]{./figure/temporal_dependency_different_day.png}
        }
    
    }
    %\caption{Temporan dependency of a region in two days~(08:00 ~ 20:00): The region has higher short-term dependency on February, 21, 2005 than February, 20, 2005 because of the extreme weather in New York city on February, 21, 2005.}
    \caption{Temporal dependency of different regions and on different days.}
    %\label{fig:anomaly effect on temporal dependency dependency}
    \end{figure}


    

\begin{figure}
    \noindent\makebox[\linewidth][c]{
        \subfigure[February, 20, 2005]{
            \label{fig:20150220}
            \includegraphics[width=0.25\textwidth]{./figure/temporal_dependency_20150220.png}
        }
        \vspace{.6in}
        \subfigure[February, 21, 2005]{
            \label{fig:20150221}
            \includegraphics[width=0.25\textwidth]{./figure/temporal_dependency_20150221.png}
        }
    
    }
    %\caption{Temporan dependency of a region in two days~(08:00 ~ 20:00): The region has higher short-term dependency on February, 21, 2005 than February, 20, 2005 because of the extreme weather in New York city on February, 21, 2005.}
    \caption{Temporal dependency of a region at different time slots~(8:00 - 20:00) on February, 21, 2005 and February, 21, 2005.}
    \label{fig:anomaly effect on temporal dependency dependency}
    \end{figure}


Then, we demonstrate the temporal dependencies of the same region at the same time-of-day on different days in Figure \ref{fig:different day}. The x-axis is the $16$ historical time slots, and the y-axis represents the same time-of-day of $10$ different days. We find that even for the same region at the same time-of-day, its dependency on the historical time slot is different on distinct days.
Moreover, we show the temporal dependencies of the same region at different time slots on Feb, 20, 2015~(Figure \ref{fig:20150220}) and Feb, 21, 2015~(Figure \ref{fig:20150221}). The x-axis is the $16$ historical time slots while the y-axis is $24$ different time slots~(08:00 - 20:00) in a day. The figures show that the temporal dependency of a region not only varies on different days but also at different time slots on the same day. The results in Figures \ref{fig:different day} and \ref{fig:anomaly effect on temporal dependency dependency} are consistent with our common sense: the traffic of a region is significantly dynamic over time, and its temporal dependency hence varies. The results demonstrate that our \FRAMEWORK{} has the capacity to capture the dynamic temporal dependencies over time. 

Furthermore, we find that the color when $x = {0,1,\cdots,5}$ in Figure \ref{fig:20150221} is darker than in Figure \ref{fig:20150220}, indicating that the short-term dependency is more significant on Feb 21 than on Feb 20. The reason is that there was a snow and ice event on Feb 21\footnote{https://www.weather.gov/okx/stormevents}. Such extreme weather negatively influences the periodical modeling, so our model focuses more on the short-term dependency for Feb 21. The result demonstrates that even without external data, \FRAMEWORK{} can consider the irregularity effect by comparing the embedding of $t$ with historical time slots, and assigning different weights for the time slots.












